Inferring Pitch from Coarse Spectral Features

Fundamental frequency (F0) has long been treated as the physical definition of "pitch" in phonetic analysis. But there have been many demonstrations that F0 is at best an approximation to pitch, both in production and in perception: pitch is not F0, and F0 is not pitch. Changes in the pitch involve many articulatory and acoustic covariates; pitch perception often deviates from what F0 analysis predicts; and in fact, quasi-periodic signals from a single voice source are often incompletely characterized by an attempt to define a single time-varying F0. In this paper, we find strong support for the existence of covariates for pitch in aspects of relatively coarse spectra, in which an overtone series is not available. Thus linear regression can predict the pitch of simple vocalizations, produced by an articulatory synthesizer or by human, from single frames of such coarse spectra. Across speakers, and in more complex vocalizations, our experiments indicate that the covariates are not quite so simple, though apparently still available for more sophisticated modeling. On this basis, we propose that the field needs a better way of thinking about speech pitch, just as celestial mechanics requires us to go beyond Newton's point mass approximations to heavenly bodies.

==> 07-candidate_figures.tex <==
\section{Candidate figures}
\label{sec:cand}
\begin{figure}[h!tb]
		\centering
		  \subfigure[Train on male, Test on female]{
			\centering	\includegraphics[width=\linewidth]{Figures/Linear_train_male_full_female_stimuli_extra_to_plot_pitch.png}
			\label{fig:train_m_test_f}}\\[-1ex]
		  \subfigure[Train on female, Test on male]{
			\centering	\includegraphics[width=\linewidth]{Figures/Linear_train_female_full_male_stimuli_extra_to_plot_pitch.png}
			\label{fig:train_f_test_m}}
\caption{Pitch prediction when the training and test speakers are different.}
\label{fig:mismatch}
\end{figure}

\begin{table*}[th]
  \caption{Normalized root-mean-square error of regression for each parameter.}
  \label{tab:rmse_four_param_landscape}
  \centering
  \begin{tabular}{c||cccc}
    \toprule
    \textbf{Parameters} & \textbf{Frequency (F0)} 
    & \textbf{Tenseness} 
    & \textbf{Tongue\_diameter}
    & \textbf{Tongue\_index}
    \\
    \midrule
    Training & 0.0060 & 0.2016 & 0.2198 & 0.0561 \\\hline
    Test & 0.0097 & 0.2650 & 0.2427 & 0.0616 \\
    \bottomrule
  \end{tabular}
\end{table*}

\begin{figure*}[h!tb]
		\centering
		  \subfigure[Train on male, Test on female]{
			\centering	\includegraphics[width=0.48\linewidth]{Figures/Linear_train_male_full_female_stimuli_extra_to_plot_pitch.png}
			\label{fig:train_m_test_f}}
		  \subfigure[Train on female, Test on male]{
			\centering	\includegraphics[width=0.48\linewidth]{Figures/Linear_train_female_full_male_stimuli_extra_to_plot_pitch.png}
			\label{fig:train_f_test_m}}
\caption{Pitch prediction when the training and test speakers are different.}
\label{fig:mismatch}
\end{figure*}

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.75\linewidth]{Figures/pitch_f0.pdf}
\caption{Relationship between pitch and F0.}
\label{fig:pitch_f0}
\end{figure}

\begin{figure}[htp]
	\centering
	\includegraphics[width=\linewidth]{Figures/RMSE_corr_MLP_semitone.pdf}
\caption{The RMSE and Pearson correlation between the gold pitch and predicted pitch based on the amount of training data. Full training data is \textbf{4 minutes}. Results from two regression models are presented. Linear regression is in circle marker, while Multi-layper Perceptron (MLP) regressor is in triangle.}
\label{fig:rmse_corr_mlp}
\end{figure}

\begin{figure*}[htb]
		\centering
		  \subfigure[Train on one vowel one speaker]{
			\centering	\includegraphics[width=0.51\linewidth]{Figures/6x6_RMSE_total_semitone_heatmap.pdf}
			\label{fig:6x6_rmse}}
			\hspace{-3em}
		  \subfigure[Train on all the vowel stimuli]{
			\centering	\includegraphics[width=0.51\linewidth]{Figures/expand_RMSE_heatmap_semitone.pdf}
			\label{fig:expand_rmse}}\\[-1ex]
\caption{Root-mean-square error (RMSE) between gold and the predicted pitch. Each cell represents one training/test set combination. ``F'' and ``M'' represent female and male speakers respectively. Lighter colors indicate lower error. (a) shows RMSE when the training data is one vowel stimuli from one speaker, whereas (b) shows the result when the training data is all the vowel stimuli from either speaker or from both speakers.}
\label{fig:rmse_cm}
\end{figure*}

\begin{figure}[htb]
        %\begin{minipage}{0.35\textwidth}
        \subfigure[Pitch]{
			\centering
			\includegraphics[width=\linewidth]{Figures/ii_excerpt_to_plot_pitch.pdf}
			\label{fig:female_pitch}}\\[-1ex]
		\centering
		 	\subfigure[MFCC]{
			\centering
			\includegraphics[width=\linewidth]{Figures/ii_excerpt_to_plot_MFCC.pdf}
			\label{fig:female_mfcc}}\\[-2ex]
        %\hspace{0.01in}
        	\subfigure[Spectrogram]{
			\centering
			\includegraphics[width=\linewidth]{Figures/ii_excerpt_to_plot_spectrogram.pdf}
			\label{fig:female_spec}}\\
        %\hspace{0.01in}
		\caption{The pitch tracks, MFCCs, and spectrogram of a test sample from the female speaker. (a) is pitch tracks from Praat. (b) is a plot of normalized 40-D MFCCs. (c) is narrow-band spectrogram, where the window length is set to 30ms, pre-emphasis is 0dB/oct and dynamic range is 80dB.}
		\label{fig:hodgepodge}
\end{figure}

\begin{figure*}[h!tb]
        %\begin{minipage}{0.35\textwidth}
		\centering
		    \subfigure[Female pitch.]{
			\centering
			\includegraphics[scale=0.33]{Figures/ii_excerpt_to_plot_pitch.pdf}
			\label{fig:female_pitch}}
		\hspace{-2em}
		 	\subfigure[Female MFCC.]{
			\centering
			\includegraphics[scale=0.33]{Figures/ii_excerpt_to_plot_MFCC.pdf}
			\label{fig:female_mfcc}}
        \hspace{-2em}
        	\subfigure[Female spectrogram.]{
			\centering
			\includegraphics[scale=0.5]{Figures/ii_excerpt_to_plot_spectrogram.pdf}
			\label{fig:female_spec}}\\[-1ex]
        %\hspace{0.01in}
        %\end{minipage}
        %\begin{minipage}{0.35\textwidth}
            \subfigure[Male pitch.]{
			\centering
			\includegraphics[scale=0.33]{Figures/male_ii_to_plot_pitch.pdf}
			\label{fig:male_pitch}}
		\hspace{-2em}
		    \subfigure[Male MFCC.]{
			\centering
			\includegraphics[scale=0.33]{Figures/male_ii_to_plot_MFCC.pdf}
			\label{fig:male_mfcc}}
		\hspace{-2em}
        	\subfigure[Male spectrogram.]{
			\centering
			\includegraphics[scale=0.5]{Figures/male_ii_to_plot_spectrogram.pdf}
			\label{fig:male_spec}}\\[-1ex]
        %\hspace{0.01in}\\
            \subfigure[Correlation between F0 and MFCC for the female speaker.]{
			\centering
			\includegraphics[width=0.4\linewidth]{Figures/female_corr_mfcc.pdf}
			\label{fig:female_corr}}
% 		\hspace{-2em}
		    \subfigure[Correlation between F0 and MFCC for the male speaker.]{
			\centering
			\includegraphics[width=0.4\linewidth]{Figures/male_corr_mfcc.pdf}
			\label{fig:male_corr}}\\[-1ex]
		\caption{An overview of human stimuli. (a)-(c) are representing a 5-second excerpt of audio data from the female speaker, and (d)-(f) are representing that of the male speaker. Both examples are utterances of the vowel /\textipa{i}/. (a) and (d) are pitch tracks from Praat. (b) and (e) are plots of normalized 40-D MFCCs. (c) and (f) are narrow-band spectrograms, where the window length is set to 30ms, pre-emphasis is 0dB/oct and dynamic range is 80dB. (g) and (h) are the Pearson correlation coefficient between F0 and each dimension of cepstral coefficients. The correlation is obtained from all the vowel stimuli collected from each speaker.}
		\label{fig:hodgepodge}
\end{figure*}

\begin{figure*}[htp]
	\centering
		\subfigure[Train on one vowel one speaker]{
		\centering	\includegraphics[width=0.48\linewidth]{Figures/6x6_RMSE_total_heatmap.pdf}
		\label{fig:four_6x6_rmse}}
		\hspace{-3em}
    \subfigure[Train on one vowel one speaker]{
	\centering	\includegraphics[width=0.48\linewidth]{Figures/6x6_corr_total_heatmap.pdf}
	\label{fig:four_6x6_corr}}
	\hspace{-3em}
  \subfigure[Train on all the vowel stimuli]{
	\centering	\includegraphics[width=0.48\linewidth]{Figures/expand_RMSE_heatmap.pdf}
	\label{fig:four_expand_rmse}}
	\hspace{-3em}
    \subfigure[Train on all the vowel stimuli]{
	\centering	\includegraphics[width=0.48\linewidth]{Figures/expand_corr_heatmap.pdf}
	\label{fig:four_expand_corr}}
\caption{Pearson correlation between the predicted pitch and the gold pitch. Each cell represents one train/test set combination. ``F'' and ``M'' represents female and male speaker respectively. Lighter colors indicate stronger positive correlation. $\triangle$ on a cell means the result is \textbf{not} statistically significant (p $>$ 0.05). (a) shows the result when the training data is one vowel stimuli from one speaker, whereas (b) shows the result when the training data is all the vowel stimuli from either speaker and from both speakers.}
\label{fig:four_corr_cm}
\end{figure*}
